Stochastic Primal Dual Hybrid Gradient Algorithm with Adaptive Step-Sizes

In this work we propose a new primal-dual algorithm with adaptive step-sizes. The stochastic primal-dual hybrid gradient (SPDHG) algorithm with constant step-sizes has become widely applied in large-scale convex optimization across many scientific fields due to its scalability. While the product of the primal and dual step-sizes is subject to an upper-bound in order to ensure convergence, the selection of the ratio of the step-sizes is critical in applications. Up-to-now there is no systematic and successful way of selecting the primal and dual step-sizes for SPDHG. In this work, we propose a general class of adaptive SPDHG (A-SPDHG) algorithms, and prove their convergence under weak assumptions. We also propose concrete parameters-updating strategies which satisfy the assumptions of our theory and thereby lead to convergent algorithms. Numerical examples on computed tomography demonstrate the effectiveness of the proposed schemes.

==> backup_texs.tex <==




\begin{figure}[t]
   \centering
      \subfloat[starting ratio $10^{-1}$ ]{\includegraphics[width= .475\textwidth]{figs/a_i2e1.eps}}
      \subfloat[starting ratio $10^{-3}$ ]{\includegraphics[width= .475\textwidth]{figs/a_i2e3.eps}}\\
    \subfloat[starting ratio $10^{-5}$ ]{\includegraphics[width= .475\textwidth]{figs/a_i2e5.eps}}
      \subfloat[starting ratio $10^{-7}$ ]{\includegraphics[width= .475\textwidth]{figs/a_i2e7.eps}}\\
   \caption{Comparison between SPDHG and our A-SPDHG on X-ray fanbeam CT example, with a variety of starting primal-dual step-size ratios. We can observe that the ideal ratio in this example is around $10^{-5}$, and our A-SPDHG algorithm is able to adjust the step-size ratio to this optimal regime regardless of the starting ratio, and achieves improved performance over SPDHG.}
\label{f1}
\end{figure}

\begin{figure}[t]
   \centering

      \subfloat[starting ratio $10^{-1}$ ]{\includegraphics[width= .475\textwidth]{figs/a_i1e1.eps}}
      \subfloat[starting ratio $10^{-3}$ ]{\includegraphics[width= .475\textwidth]{figs/a_i1e3.eps}}\\
    \subfloat[starting ratio $10^{-5}$ ]{\includegraphics[width= .475\textwidth]{figs/a_i1e5.eps}}
      \subfloat[starting ratio $10^{-7}$ ]{\includegraphics[width= .475\textwidth]{figs/a_i1e7.eps}}\\
   \caption{Comparison between SPDHG and our A-SPDHG on X-ray fanbeam CT example, with a variety of starting primal-dual step-size ratios. We can observe that the ideal ratio in this example is around $10^{-5}$, and our A-SPDHG algorithm is able to adjust the step-size ratio to this optimal regime regardless of the starting ratio, and achieves improved performance over SPDHG.}
\label{f2}
\end{figure}




\begin{figure}[t]
   \centering

      \subfloat[Test on the choices for $\alpha_0$ ]{\includegraphics[trim=0 230 0 0,clip,width= .475\textwidth]{figs/test_alpha.eps}}
      \subfloat[Test on the choices for $\eta$ ]{\includegraphics[trim=0 230 0 0,clip,width= .475\textwidth]{figs/test_param_eta.eps}}\\
    \subfloat[Test on the choices for $s$ ]{\includegraphics[trim=0 230 0 0,clip,width= .475\textwidth]{figs/test_ss.eps}}
      \subfloat[Test on the choices for $\delta$ ]{\includegraphics[trim=0 230 0 0,clip,width= .475\textwidth]{figs/test_del.eps}}\\
   \caption{Test on different choices of parameters of A-SPDHG (rule-a) on X-ray fanbeam CT example, starting ratio of primal-dual step-sizes: $10^{-3}$.}
\label{f3}
\end{figure}


%trim=0 250 0 0,clip,
\begin{figure}[t]
   \centering

      \subfloat[Test on the choices for $c$ ]{\includegraphics[width= .475\textwidth]{figs/test_c.eps}}
      \subfloat[Test on the choices for $\eta$ ]{\includegraphics[width= .475\textwidth]{figs/test_b_eta.eps}}
   \caption{Test on different choices of parameters of A-SPDHG (rule-b) on X-ray fanbeam CT example, starting ratio of primal-dual step-sizes: $10^{-3}$.}
\label{f4}
\end{figure}
